Peak-Detector: Explainable Peak Detection via Instruction-Tuned Large Language Models in Physiological Sign

Accurate peak detection across diverse cardiac physiological signals, including the Electrocardiogram (ECG), Photoplethysmogram (PPG), Ballistocardiogram (BCG), and Bodyseismography (BSG), is fundamental for cardiovascular monitoring but is often hindered by artifacts and signal variability. Conventional algorithms are typically engineered with expert knowledge for a single signal modality, limiting their generalizability. Conversely, deep learning-based methods often lack interpretability, limiting transparency for expert verification and hindering expert-computer interaction. To address these limitations, we introduce Peak-Detector, a novel framework that leverages instruction-tuned Large Language Models (LLMs) for robust, cross-modal, and explainable peak detection. A core innovation of our framework is a "peak-representation" technique that transforms time-series data into a condensed format, preserving critical event information while significantly reducing signal length. This representation provides a crucial inductive bias, guiding the LLM to reason over physiologically meaningful events rather than raw, noisy data. The model is optimized through a two-stage process: supervised fine-tuning (SFT) followed by reinforcement learning (RL) with a multi-objective reward function. The model's self-explanation capabilities are cultivated by fine-tuning on a custom-built Peak-Explanation dataset. Across four modalities-ECG, PPG, BCG, and BSG-spanning seven datasets (six public benchmarks plus one real-world cohort), Peak-Detector demonstrates strong cross-modal performance, achieving best or tied-best detection under clinically relevant temporal tolerance. Beyond accuracy, the generated rationales surface failure modes and support verification and error analysis.

==> source/experiment4.7.tex <==
\subsection{Cross-Dataset Generalization Analysis}
\label{sec:Cross_Modality}

To assess the generalization capabilities and robustness of Peak-Detector to domain shift, we conducted a comprehensive cross-dataset evaluation. Models were trained on a single source dataset and evaluated on all others. The F1-score results for Peak-Detector and the strongest baseline, FR-Net, are presented in Table~\ref{tab:cross_domain} and Table~\ref{tab:cross_domain_FRnet}, respectively.

\textbf{In-Domain Analysis.}
When evaluated on an in-domain but unseen dataset (e.g., training on MIT-BIH and testing on Incart), Peak-Detector's F1-score drops slightly from 0.9805 to 0.9580. This minor degradation, observed across all modalities, suggests that while the model learns modality-specific features effectively, it is also susceptible to dataset-specific biases, even within the same signal type.



\begin{table}[htbp!]
\centering
\caption{Cross-Dataset Generalization Performance (F1-score) for Peak-Detector. Rows indicate the training (source) dataset and columns indicate the testing (target) dataset.}
\label{tab:cross_domain}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{l|cccccc}
\toprule
\textbf{Source / Target} & \textbf{MIT-BIH} & \textbf{Incart} & \textbf{BIDMC} & \textbf{Capnobase} & \textbf{Kansas} & \textbf{BCG Arry.} \\
\midrule
\textbf{MIT-BIH} & 0.9729 & 0.9580 & 0.6304 & 0.7466 & 0.4401 & 0.6440 \\
\textbf{Incart} & 0.9677 & 0.9805 & 0.2550 & 0.4494 & 0.3002 & 0.5376 \\
\textbf{BIDMC} & 0.3597 & 0.3726 & 0.9928 & 0.9564 & 0.3410 & 0.8040 \\
\textbf{Capnobase} & 0.4871 & 0.4129 & 0.9380 & 0.9912 & 0.3141 & 0.5957 \\
\textbf{Kansas} & 0.4217 & 0.5672 & 0.8656 & 0.8592 & 0.9544 & 0.8912 \\
\textbf{BCG Arry.} & 0.4230 & 0.5337 & 0.8639 & 0.7218 & 0.7556 & 0.9545 \\
\hline
\textbf{Combined Model} & 0.9681 & 0.9342 & 0.9877 & 0.9142 & 0.9379 & 0.8930 \\
\bottomrule
\end{tabular}}
\end{table}

% \vspace{-5mm}
\begin{table}[h!]
\centering
\caption{Cross-Dataset Generalization Performance (F1-score) for FR-Net. Rows indicate the training (source) dataset and columns indicate the testing (target) dataset.}
\label{tab:cross_domain_FRnet}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{l|cccccc}
\toprule
\textbf{Source / Target} & \textbf{MIT-BIH} & \textbf{Incart} & \textbf{BIDMC} & \textbf{Capnobase} & \textbf{Kansas} & \textbf{BCG Arry.} \\
\midrule
\textbf{MIT-BIH} & 0.9802 & 0.8760 & 0.8436 & 0.1005 & 0.6273 & 0.8683 \\
\textbf{Incart} & 0.9570 & 0.9897 & 0.6838 & 0.0019 & 0.1070 & 0.5477 \\
\textbf{BIDMC} & 0.4312 & 0.3859 & 0.9679 & 0.9870 & 0.5050 & 0.8151 \\
\textbf{Capnobase} & 0.2320 & 0.0966 & 0.9458 & 0.9844 & 0.3229 & 0.2982 \\
\textbf{Kansas} & 0.6329 & 0.6717 & 0.8565 & 0.8858 & 0.9230 & 0.8795 \\
\textbf{BCG Arry.} & 0.8460 & 0.7228 & 0.8765 & 0.7792 & 0.8088 & 0.9120 \\
\hline
\textbf{Combined Model} & 0.9690 & 0.8816 & 0.8688 & 0.2467 & 0.9347 & 0.8879 \\
\bottomrule
\end{tabular}}
\end{table}

\textbf{Cross-Domain Analysis.}
Performance degrades more significantly in cross-domain scenarios, highlighting that models learn features specific to the physiological origin of each modality (electrical vs. optical vs. mechanical). For instance, Peak-Detector trained on ECG data (MIT-BIH) achieves an F1-score of 0.6304 when tested on PPG data (BIDMC). Crucially, even this attenuated performance is substantially higher than that of an untrained base model (F1-score of 0.1712, see Table~\ref{tab:ablation_study}), indicating that the framework learns a foundational, transferable knowledge of what constitutes a "peak." In comparison, FR-Net suffers a far more severe performance degradation in similar scenarios. When trained on MIT-BIH (ECG) and tested on Capnobase (PPG), FR-Net’s F1-score plummets to 0.1005, a near-total failure. In the same scenario, Peak-Detector maintains a functional F1-score of 0.7466. This stark difference suggests that while FR-Net excels at learning modality-specific features, its representations are less transferable, whereas Peak-Detector's language-based reasoning provides greater out-of-domain robustness.

\textbf{Performance of a Combined Model.}
The most compelling evidence for our framework's potential as a universal peak detector is the performance of the Combined Model, trained on a mixed dataset (MIT-BIH, BIDMC, and Kansas). As shown in the final row of Table~\ref{tab:cross_domain}, this single model achieves robust and high-quality performance across all six test sets, closely approaching the results of the specialized, individually trained models (e.g., 0.9877 on BIDMC vs. 0.9928 for the specialized model). In contrast, the combined FR-Net model exhibits poor generalization. While it performs well on the modalities included in its mixed training (ECG and BCG), its performance on the unseen PPG datasets is significantly worse than that of a specialized PPG-trained FR-Net (e.g., an F1-score of 0.2467 on Capnobase, compared to 0.9844 for the specialized model). This outcome strongly suggests that the Peak-Detector framework can be effectively scaled with diverse data to create a single, powerful, and truly generalizable model for cross-modal analysis—a capability not demonstrated by the conventional deep learning architecture.

==> source/future_work.tex <==
\section{Future Work}


The findings of this study indicate several critical directions for advancing the field of ballistocardiography-based blood pressure estimation. We outline below the principal methodological and translational opportunities that warrant systematic investigation.

\subsection{Context-Aware and Multimodal Prediction}

The current PULSE-MoE framework relies exclusively on features extracted from the BSG/BCG signal. However, blood pressure regulation is inherently multifactorial, and significant inter- and intra-patient variability can arise from demographic, postural, and environmental factors. Future research should rigorously evaluate the integration of contextual information—such as age, sex, body position, and clinical history—as well as additional physiological signals (e.g., ECG, PPG, accelerometry). The incorporation of such multimodal data is expected to enhance the discriminative capacity of predictive models, improve generalizability across heterogeneous cohorts, and enable the development of personalized monitoring systems.

\subsection{Robust Physiological Signal Characterization}

PULSE-MoE utilizes heuristic-based peak detection for the extraction of physiological features such as J-K interval and heart rate variability. This methodology is susceptible to noise and may exhibit reduced reliability under the suboptimal signal conditions typical of ICU environments. Future work should focus on the development of advanced signal processing pipelines and data-driven feature extraction methods, including deep neural networks trained for robust identification of physiologically meaningful patterns amidst noise and artifact. The adoption of such techniques could substantially improve the accuracy and reliability of feature extraction, thereby enhancing downstream prediction performance.

\subsection{Interpretability and Physiological Model Integration}

Interpretability remains essential for the clinical acceptance and regulatory approval of machine learning-based monitoring systems. Beyond accurate blood pressure estimation, future modeling efforts should prioritize the development of mechanisms to elucidate the physiological basis of predictions and to provide transparent reasoning for model outputs. Methods such as attention-based interpretability, post hoc attribution analyses, and the incorporation of explicit physiological knowledge or constraints into model architectures should be systematically explored. Furthermore, expanding the modeling framework to jointly estimate related hemodynamic or diagnostic states may provide synergistic gains in both accuracy and clinical relevance.
